Deviation results for Mandelbrot's multiplicative cascades with exponential tails

Let $W$ be a nonnegative random variable with expectation $1$. For all $r \geqslant 2$, we consider the total mass $Z_r^\infty$ of the associated Mandelbrot multiplicative cascade in the $r$-ary tree. For all $n \geqslant 1$, we also consider the total mass $Z_r^n$ of the measure at height $n$ in the $r$-ary tree. Liu, Rio, Rouault \cite{lrr,liu2000limit,Rouault04} established large deviation results for $(Z_r^n)_{r \geqslant 2}$ for all $n \in [[1,\infty[[$ (resp., for $n = \infty$) in case $W$ has an everywhere finite cumulant generating function $\Lambda_W$ (resp., $W$ is bounded). Here, we extend these results to the case where $\Lambda_W$ is only finite on a neighborhood of zero. And we establish all deviation results (moderate, large, and very large deviations). It is noticeable that we obtain nonconvex rate functions. Moreover, our proof of upper bounds of deviations for $(Z_r^\infty)_{r \geqslant 2}$ rely on the moment bound instead of the standard Chernoff bound.

==> commath.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Commandes mathématiques
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\RequirePackage{babel}					%Pour les commandes dépendant de la langue du document
\RequirePackage{amsmath}				%Math de l'AMS
\RequirePackage{amssymb}				%Autres symboles mathématiques
\RequirePackage{amsthm}					%Théorèmes correctement organisés
\RequirePackage{bbm}					%Fonction indicatrice
\RequirePackage{stmaryrd}				%Crochets pour les intervalles entiers

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Rémi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% Making \big, etc. a relative size rather than absolute (with default parameters, ex is 4.3045 pt)
%
%\renewcommand\big[1]{{\hbox{$\left#1\vbox to 1.97ex{}\right.\n@space$}}}
%\renewcommand\Big[1]{{\hbox{$\left#1\vbox to 2.67ex{}\right.\n@space$}}}
%\renewcommand\bigg[1]{{\hbox{$\left#1\vbox to 3.37ex{}\right.\n@space$}}}
%\renewcommand\Bigg[1]{{\hbox{$\left#1\vbox to 4.07ex{}\right.\n@space$}}}
%
%% Paired delimiters
%
%\DeclarePairedDelimiter\abs\lvert\rvert % Absolute value
%\DeclarePairedDelimiter\brack\lbrack\rbrack % Brackets
%\DeclarePairedDelimiter\ceil\lceil\rceil % Ceiling
%\DeclarePairedDelimiter\floor\lfloor\rfloor % Floor
%\DeclarePairedDelimiter\intervalicc\llbracket\rrbracket % Closed integer interval
%\DeclarePairedDelimiter\intervalico\llbracket\llbracket % Closed-open integer interval
%\DeclarePairedDelimiter\intervalioc\rrbracket\rrbracket % Open-closed integer interval
%\DeclarePairedDelimiter\intervalioo\rrbracket\llbracket % Open interger interval
%\DeclarePairedDelimiter\norm\lVert\rVert % Norm
%\DeclarePairedDelimiter\paren() % Parentheses
%\DeclarePairedDelimiter\set\{\} % Set
%
%\DeclarePairedDelimiterX\inner[2]\langle\rangle{#1,#2} % Inner product
%\DeclarePairedDelimiterX\intervalcc[2]\lbrack\rbrack{#1,#2} % Closed interval
%\DeclarePairedDelimiterX\intervalco[2]\lbrack\rparen{#1,#2} % Closed-open interval
%\DeclarePairedDelimiterX\intervaloc[2]\lparen\rbrack{#1,#2} % Open-closed interval
%\DeclarePairedDelimiterX\intervaloo[2]\lparen\rparen{#1,#2} % Open interval
%\DeclarePairedDelimiterX\setst[2]\{\}{#1\ \delimsize|\ #2} % Set of the #1 such that #2
%
%% Use of some characters from the Fourier-GUTenberg package
%
%\DeclareFontEncoding{FMS}{}{}
%\DeclareFontSubstitution{FMS}{futm}{m}{n}
%\DeclareFontEncoding{FMX}{}{}
%\DeclareFontSubstitution{FMX}{futm}{m}{n}
%\DeclareSymbolFont{fouriersymbols}{FMS}{futm}{m}{n}
%\DeclareSymbolFont{fourierlargesymbols}{FMX}{futm}{m}{n}
%\DeclareMathDelimiter{\llbracket}{\mathopen}{fouriersymbols}{153}{fourierlargesymbols}{133}
%\DeclareMathDelimiter{\rrbracket}{\mathclose}{fouriersymbols}{154}{fourierlargesymbols}{134}
%\DeclareMathDelimiter{\VERT}{\mathord}{fouriersymbols}{152}{fourierlargesymbols}{147}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Mathématiques générales
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%Ensembles de nombres
\newcommand{\ensnombre}[1]{\mathbb{#1}}%
\newcommand{\N}{\ensnombre{N}}
\newcommand{\Z}{\ensnombre{Z}}
\newcommand{\Q}{\ensnombre{Q}}
\newcommand{\R}{\ensnombre{R}}
\newcommand{\C}{\ensnombre{C}}

%Divers
\newcommand{\card}[1]{\left\lvert #1 \right\rvert}

\DeclareMathOperator{\id}{id}
\DeclareMathOperator{\dom}{dom}

\renewcommand{\Re}{\mathfrak{Re}}
\renewcommand{\Im}{\mathfrak{Im}}

\newcommand{\abs}[1]{\left\lvert #1 \right\rvert}
\newcommand{\norme}[1]{\left\lVert #1 \right\rVert}
\newcommand{\prodscal}[2]{\left\langle {#1} \mathrel{}\middle|\mathrel{} {#2} \right\rangle}
\newcommand{\floor}[1]{\left\lfloor #1 \right\rfloor}
\newcommand{\ceil}[1]{\left\lceil #1 \right\rceil}

\newcommand{\ensfonction}[3]{#1(#2 ; #3)}
\newcommand{\enstq}[2]{\left\{ #1 \mathrel{}\middle|\mathrel{} #2 \right\}}
\newcommand{\ensavec}[2]{\left\{ #1\ ;\ #2 \right\}}
\newcommand{\enspart}{\mathfrak{P}}

\newcommand{\defeq}{\mathrel{\mathop:}=}
\newcommand{\eqdef}{\mathrel{=}:}

\newcommand{\seq}[1]{#1}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Algèbre linéaire
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\ensmatrice}[3]{\mathcal{#1}_{#2}(#3)}

\newcommand{\transposee}[1]{{#1}^\top}
%\newcommand{\transposee}[1]{{}^t\! #1}

\DeclareMathOperator{\rg}{rg}
\DeclareMathOperator{\Ima}{Im}
\DeclareMathOperator{\Ker}{Ker}
\DeclareMathOperator{\Dom}{Dom}
\DeclareMathOperator{\tr}{tr}
\DeclareMathOperator{\Com}{Com}
\DeclareMathOperator{\Mat}{Mat}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Probabilités
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\indic}{\mathbbm{1}}
\DeclareMathOperator{\Leb}{Leb}
\newcommand{\Prob}{\mathbb{P}}
\newcommand{\Loi}{\mathcal{L}}
\newcommand{\Espe}{\mathbb{E}}
\newcommand{\ET}{\sigma}
\DeclareMathOperator{\Var}{Var}
\DeclareMathOperator{\Cov}{Cov}
\newcommand{\complementaire}[1]{#1^\mathsf{c}}

\newcommand{\Probcond}[2]{\Prob\left( #1 \mathrel{}\middle|\mathrel{} #2 \right)}
\newcommand{\Loicond}[2]{\Loi\left(#1 \mathrel{}\middle|\mathrel{} #2 \right)}
\newcommand{\Especond}[2]{\Espe\left[ #1 \mathrel{}\middle|\mathrel{} #2 \right]}
\newcommand{\Varcond}[2]{\Var\left(#1 \mathrel{}\middle|\mathrel{} #2 \right)}




\iflanguage{french}%
{
%VERSION FRANCAISE

\DeclareMathOperator{\Vect}{Vect}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Fonctions
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\let\cosh\relax
\DeclareMathOperator{\cosh}{ch}
\let\sinh\relax
\DeclareMathOperator{\sinh}{sh}
\let\tanh\relax
\DeclareMathOperator{\tanh}{th}

\DeclareMathOperator{\cotan}{cotan}
\DeclareMathOperator{\sinc}{sinc}
\DeclareMathOperator{\arcosh}{argch}
\DeclareMathOperator{\arsinh}{argsh}
\DeclareMathOperator{\artanh}{argth}

\DeclareMathOperator{\argmin}{argmin}
\DeclareMathOperator*{\supess}{sup\,ess}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Intervalles
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\newcommand{\intervalle}[4]{\left#1#2\mathclose{}\mathpunct{};#3\right#4}%
\newcommand{\intervalle}[4]{\left#1#2\mathclose{},#3\right#4}%
\newcommand{\intervalleff}[2]{\intervalle{[}{#1}{#2}{]}}%
\newcommand{\intervalleof}[2]{\intervalle{]}{#1}{#2}{]}}%
\newcommand{\intervallefo}[2]{\intervalle{[}{#1}{#2}{[}}%
\newcommand{\intervalleoo}[2]{\intervalle{]}{#1}{#2}{[}}%
\newcommand{\intervallentff}[2]{\intervalle{\llbracket}{#1}{#2}{\rrbracket}}%
\newcommand{\intervallentof}[2]{\intervalle{\rrbracket}{#1}{#2}{\rrbracket}}%
\newcommand{\intervallentfo}[2]{\intervalle{\llbracket}{#1}{#2}{\llbracket}}%
\newcommand{\intervallentoo}[2]{\intervalle{\rrbracket}{#1}{#2}{\llbracket}}%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Théorèmes
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\theoremstyle{plain}%
\newtheorem{theorem}{Théorème}%
\newtheorem{lemma}{Lemme}%
%\newtheorem{lemma}[theorem]{Lemme}%
%\newtheorem{lemma}[section]{Lemme}%
\newtheorem{corollary}{Corollaire}%
\newtheorem{proposition}{Proposition}%
\newtheorem{property}{Propriété}%
\newtheorem{properties}{Propriétés}%
\newtheorem*{fact}{Fait}%
%
\theoremstyle{definition}%
\newtheorem{definition}{Définition}%
\newtheorem{hypothesis}{Hypothèse}%
\newtheorem{example}{Exemple}%
\newtheorem{examples}{Exemples}%
\newtheorem*{exercise}{Exercice}%
%
\theoremstyle{remark}%
\newtheorem*{remark}{Remarque}%
\newtheorem*{plus}{Complément}%
\newtheorem*{question}{Question}%
\theoremstyle{plain}%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Topologie
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\DeclareMathOperator{\interieur}{int}
\DeclareMathOperator{\adherence}{adh}
}
{
%VERSION ANGLAISE

\DeclareMathOperator{\Vect}{span}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Fonctions
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\DeclareMathOperator{\cotan}{cotan}
\DeclareMathOperator{\arcosh}{arcosh}
\DeclareMathOperator{\arsinh}{arsinh}
\DeclareMathOperator{\artanh}{artanh}

\DeclareMathOperator{\argmin}{argmin}
\DeclareMathOperator*{\supess}{ess\,sup}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Intervalles
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\intervalle}[4]{\left#1#2,#3\right#4}%
\newcommand{\intervalleff}[2]{\intervalle{[}{#1}{#2}{]}}%
\newcommand{\intervalleof}[2]{\intervalle{(}{#1}{#2}{]}}%
\newcommand{\intervallefo}[2]{\intervalle{[}{#1}{#2}{)}}%
\newcommand{\intervalleoo}[2]{\intervalle{(}{#1}{#2}{)}}%
\newcommand{\intervallentff}[2]{\intervalle{\llbracket}{#1}{#2}{\rrbracket}}%
\newcommand{\intervallentof}[2]{\intervalle{\rrbracket}{#1}{#2}{\rrbracket}}%
\newcommand{\intervallentfo}[2]{\intervalle{\llbracket}{#1}{#2}{\llbracket}}%
\newcommand{\intervallentoo}[2]{\intervalle{\rrbracket}{#1}{#2}{\llbracket}}%

%\newcounter{intervallent}%
%\newcommand{\intervallentff}[2]{%
%	\setcounter{intervallent}{#1}%
%	\stepcounter{intervallent}%
%	\left\{#1,\theintervallent,\dots,#2\right\}}%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Théorèmes
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\theoremstyle{plain}%
\newtheorem{theorem}{Theorem}%
\newtheorem{lemma}{Lemma}%
%\newtheorem{lemma}[theorem]{Lemme}%
%\newtheorem{lemma}[section]{Lemme}%
\newtheorem{corollary}{Corollary}%
\newtheorem{proposition}{Proposition}%
\newtheorem{property}{Property}%
\newtheorem{properties}{Properties}%
\newtheorem*{fact}{Fact}%
%
\theoremstyle{definition}%
\newtheorem{definition}{Definition}%
\newtheorem{hypothesis}{Hypothesis}%
\newtheorem{example}{Example}%
\newtheorem{examples}{Examples}%
\newtheorem*{exercise}{Exercise}%
%
\theoremstyle{remark}%
\newtheorem*{remark}{Remark}%
\newtheorem*{plus}{Plus}%
\newtheorem*{question}{Question}%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Topologie
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\DeclareMathOperator{\interieur}{int}
\DeclareMathOperator{\adherence}{cl}
}

==> packmin.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Typographie
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

	\usepackage{babel}					%Typographie

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Mathématiques
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

	\usepackage{amsmath}					%Math de l'AMS
	\usepackage{amssymb}					%Autres symboles mathématiques
	\usepackage{amsthm}					%Théorèmes correctement organisés

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Divers
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%Graphiques
	\usepackage{graphicx}				%Insérer des images
	\usepackage{color}					%Couleurs (nécessaires pour les images avec XFig)

%Programmation
	\usepackage{version}					%Commenter (notamment un environnement)

%Mise en page
	\usepackage{geometry}				%Marges
